TDOA Matrices: Algebraic Properties and their Application to Robust Denoising with Missing Data

Measuring the Time delay of Arrival (TDOA) between a set of sensors is the basic setup for many applications, such as localization or signal beamforming. This paper presents the set of TDOA matrices, which are built from noise-free TDOA measurements, not requiring knowledge of the sensor array geometry. We prove that TDOA matrices are rank-two and have a special SVD decomposition that leads to a compact linear parametric representation. Properties of TDOA matrices are applied in this paper to perform denoising, by finding the TDOA matrix closest to the matrix composed with noisy measurements. The paper shows that this problem admits a closed-form solution for TDOA measurements contaminated with Gaussian noise which extends to the case of having missing data. The paper also proposes a novel robust denoising method resistant to outliers, missing data and inspired in recent advances in robust low-rank estimation. Experiments in synthetic and real datasets show TDOA-based localization, both in terms of TDOA accuracy estimation and localization error.

==> algo1-v0.tex <==
    \begin{algorithmic}[1]
      \Require $\tilde{\TDOAMatrix}$, $k$, $\epsilon$ 
      \Ensure $\TDOAMatrix\in\TDOASETn$, $\|\mbf{S}\|_0<2k$, 
      \State $\TDOAMatrix_0=\tilde{\TDOAMatrix}$ ; $\mbf{S}_0=0$ ; $t=0$
      \While{$\|\tilde{\TDOAMatrix}-\TDOAMatrix_t-\mbf{S}_t\|_F^2/\|\tilde{\TDOAMatrix}\|_F^2>\epsilon$}
      \State $t=t+1$
      \State $\TDOAMatrix_t=(\tilde{\TDOAMatrix}-\mbf{S}_{t-1})\mbf{\hat{1}}\mbf{\hat{1}}^\top+\mbf{\hat{1}}\mbf{\hat{1}}^\top(\tilde{\TDOAMatrix}-\mbf{S}_{t-1})$
      \State $\mbf{S}_t=\mathcal{P}_{2k}(\tilde{\TDOAMatrix}-\TDOAMatrix_t)$ 
      \EndWhile
      \State\Return $\TDOAMatrix_t$, $\mbf{S}_t$
  \end{algorithmic}


==> algo2-v0.tex <==
\begin{algorithmic}[1]
  \Require $\tilde{\TDOAMatrix}$, $\mbf{L}$, $k$, $\epsilon$ 
  \Ensure $\TDOAMatrix\in\TDOASETn$, $\|\mbf{S}\|_0<2k$, 
  \State $\mbf{D_\beta}=\mbf{I}\hp\mbf{L}\mbf{L}^\top$
  \State $\mbf{Q}=(\mbf{D_\beta}+\mbf{\bar{L}})^{-1}$ \label{lin:pre-cal}
  \State $\TDOAMatrix_0=\tilde{\TDOAMatrix}$ ; $\mbf{S}_0=0$ ; $t=0$
  \While{$\|\tilde{\TDOAMatrix}-\TDOAMatrix_t-\mbf{S}_t\|_F^2/\|\tilde{\TDOAMatrix}\|_F^2<\epsilon$}
  \State $t=t+1$
  
  \State $\TDOAMatrix_t=\mbf{Q}(\mbf{L}\hp\tilde{\TDOAMatrix}-\mbf{S}_{t-1})\,\mathds{1}+\mathds{1}(\mbf{L}\hp\tilde{\TDOAMatrix}-\mbf{S}_{t-1})\mbf{Q}$
  \State $\mbf{S}_t=\mathcal{P}_{2k}(\tilde{\TDOAMatrix}-\TDOAMatrix_t)$ 
  \EndWhile
  \State\Return $\TDOAMatrix_t$, $\mbf{S}_t$
\end{algorithmic}









































==> authors.tex <==
\author{Jose~Velasco,\thanks{J.~Velasco, D.~Pizarro, \ldots, and J.~Macias-Guarasa are with the Department of Electronics, Escuela Politécnica
    Superior, University of Alcalá, 28805 Alcalá de Henares, Spain.}
  Daniel~Pizarro,
  Afsaneh Asaei,~\IEEEmembership{Member,~IEEE}, \thanks{A.~Asaei is with Idiap Research Institute and
also affiliated with École Polytechnique Fédérale de Lausanne, Switzerland.}% <-this % stops a space
 \ldots
  and~Javier~Macias-Guarasa,~\IEEEmembership{Member,~IEEE}% <-this % stops a space
\thanks{E-mails: \{jose.velasco, pizarro, \ldots, macias\}@depeca.uah.es,
  \nobreak afsaneh.asaei@idiap.ch).}% <-this % stops a space  
}


==> figure-GeometricalDetails-revised.tex <==
\begin{figure}
  \centering
  \begin{subfigure}[t]{0.26\textwidth}
%  \begin{subfigure}[t]{0.27\textwidth}
    \includegraphics[width=\textwidth]{angular2-short-improved-revised}
    \caption{\scriptsize{Positions for validation\\with simulated data.}}
    \label{fig:Simulated_positions}
  \end{subfigure}
~%add desired spacing between images, e. g. ~, \quad, \qquad,
  % \hfill etc.
  % (or a blank line to force the subfigure onto a new line)
  \begin{subfigure}[t]{0.26\textwidth}
%  \begin{subfigure}[t]{0.27\textwidth}
    \includegraphics[width=\textwidth]{positions1-short-improved-revised}
    \caption{\scriptsize{Positions for validation\\with real data.}}
    \label{fig:real_positions_short}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.4125\textwidth}
%  \begin{subfigure}[t]{0.4275\textwidth}
    \includegraphics[width=\textwidth]{micNumberingpairNaming}
    \caption{\scriptsize{Numbering scheme for microphones and naming
        notation for arrangements of pairs of microphones.}}
    \label{fig:real_positions_long}
  \end{subfigure}
  \caption{{Geometrical details for the experiments carried
      out. In
      \ref{fig:simureal_positions}.\subref{fig:Simulated_positions} and
      \ref{fig:simureal_positions}.\subref{fig:real_positions_short}  only the
    relevant room section is shown.}}
  \label{fig:simureal_positions}
\end{figure}


==> figure-GeometricalDetails-simplified.tex <==
\begin{figure}
  \centering
%   \begin{subfigure}[t]{0.26\textwidth}
% %  \begin{subfigure}[t]{0.27\textwidth}
%     \includegraphics[width=\textwidth]{angular2-short-improved-revised}
%     \caption{\scriptsize{Positions for validation\\with simulated data.}}
%     \label{fig:Simulated_positions}
%   \end{subfigure}
% ~%add desired spacing between images, e. g. ~, \quad, \qquad,
%   % \hfill etc.
%   % (or a blank line to force the subfigure onto a new line)
  \begin{subfigure}[t]{0.20\textwidth}
    \includegraphics[width=\textwidth]{positions1-short-improved-revised}
    \caption{\scriptsize{Positions for validation\\with real data.}}
    \label{fig:real_positions_short}
  \end{subfigure}
  ~
  \begin{subfigure}[t]{0.24\textwidth}
    \includegraphics[width=\textwidth]{micNumberingpairNaming}
    \caption{\scriptsize{Numbering scheme for microphones and naming
        notation for arrangements of pairs of microphones.}}
    \label{fig:real_positions_long}
  \end{subfigure}
  \caption{{Geometrical details for the experiments carried
      out. In \ref{fig:simureal_positions}.\subref{fig:real_positions_short}  only the
    relevant room section is shown.}}
  \label{fig:simureal_positions}
\end{figure}


==> figure-RoomLayout.tex <==
\begin{figure*}
  \centering
  \begin{subfigure}[t]{0.24\textwidth}
    \includegraphics[width=0.8\textwidth]{roomlayout2}
    \caption{Room layout showing the centered table, and the
      microphones arranged in two circular arrays.}
    \label{fig:RoomLayout}
  \end{subfigure}%
 % \qquad \qquad %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc.
  % (or a blank line to force the subfigure onto a new line)
  \begin{subfigure}[t]{0.17\textwidth}
    \includegraphics[width=\textwidth]{positions1-short-improved-revised}
    \caption{Positions for validation with real data.}
    \label{fig:real_positions_short}
  \end{subfigure}
\qquad
  \begin{subfigure}[t]{0.25\textwidth}
    \includegraphics[width=\textwidth]{idiap-seq45-cam2.jpg}
    \caption{ Sample of recorded video frame showing the arrays area.}
    \label{fig:RoomPicture}
  \end{subfigure}
  \caption{IDIAP Smart Meeting Room for AV16.3 recordings.}
  \label{fig:LIdiapRoom}
\end{figure*}


==> figure1-v1.tex <==
\begin{figure*}[!t]
  \centering
%  \includegraphics[width=0.48\textwidth]{MapSNR_synthetic_dn_ALL_10mics.eps}
  \includegraphics[width=.7\textwidth]{MapSNR_synthetic_dn_ALL_10mics.eps}
  \caption{Robust denoising in synthetic data: SNR in dB, higher is better.}
  \label{fig:MapSNR_synthetic_dn_10mics}
\end{figure*}


==> figure1-v2.tex <==
%% \begin{wrapfigure}[19]{L}{0.7\textwidth}
%% %  \centering
%%   \includegraphics[width=0.7\textwidth]{MapSNR_synthetic_dn_ALL_10mics.eps}
%%   \caption{Robust denoising in synthetic data: SNR in dB, higher is better.}
%%   \label{fig:MapSNR_synthetic_dn_10mics}
%% \end{wrapfigure}

\begin{wrapfigure}[19]{l}[\dimexpr\columnwidth+\columnsep\relax]{12cm}
  \includegraphics[width=12cm,height=16\baselineskip]{MapSNR_synthetic_dn_ALL_10mics.eps}
  \caption{Robust denoising in synthetic data: SNR in dB, higher is better.}
  \label{fig:MapSNR_synthetic_dn_10mics}
\end{wrapfigure}


==> figure2-v1.tex <==
\begin{figure*}[!t]
  \centering
%  \includegraphics[width=0.48\textwidth]{MapCHAN_synthetic_dn_ALL_10mics.eps}
  \includegraphics[width=.7\textwidth]{MapCHAN_synthetic_dn_ALL_10mics.eps}
  \caption{Robust denoising in synthetic data: Localization error in mm (using
    \cite{chan1994simple}), lower is better.}
  \label{fig:MapCHAN_synthetic_dn_10mics}
\end{figure*}


==> figure5.tex <==
\begin{figure*}[!t]
  \centering 
  \begin{subfigure}[t]{0.18\textwidth}
    \includegraphics[width=\textwidth]{SNR_synthetic_comparative_sigma001_noutliers2_10mics}
    \caption{SNR with low noise and 2 outliers}
    \label{fig:SNR_synth_low_few}
  \end{subfigure}
\;
  \begin{subfigure}[t]{0.18\textwidth}
    \includegraphics[width=\textwidth]{SNR_synthetic_comparative_sigma001_noutliers6_10mics}
    \caption{SNR with low noise and 6 outliers}
    \label{fig:SNR_synth_low_many}
  \end{subfigure}

  \begin{subfigure}[t]{0.18\textwidth}
    \includegraphics[width=\textwidth]{SNR_synthetic_comparative_sigma200_noutliers2_10mics}
    \caption{SNR with high noise and 2 outliers}
    \label{fig:SNR_synth_high_few}
  \end{subfigure}
\;
  \begin{subfigure}[t]{0.18\textwidth}
    \includegraphics[width=\textwidth]{SNR_synthetic_comparative_sigma200_noutliers6_10mics}
    \caption{SNR with high noise and 6 outliers}
    \label{fig:SNR_synth_high_many}
  \end{subfigure}
  \begin{subfigure}[t]{0.18\textwidth}
    \includegraphics[width=\textwidth]{legend}
  \end{subfigure}

  \caption{Algorithm evaluation in synthetic data: SNR in dB.}
  \label{fig:SNR_comparative_synth}
\end{figure*}


==> figure6.tex <==
\begin{figure*}[!t]
  \centering 
  \begin{subfigure}[t]{0.18\textwidth}
    \includegraphics[width=\textwidth]{Error_synthetic_comparative_sigma001_noutliers2_10mics}
    \caption{Localization error with low noise and 2 outliers}
    \label{fig:Error_synth_low_few}
  \end{subfigure}
\;
  \begin{subfigure}[t]{0.18\textwidth}
    \includegraphics[width=\textwidth]{Error_synthetic_comparative_sigma001_noutliers6_10mics}
    \caption{Localization error with low noise and 6 outliers}
    \label{fig:Error_synth_low_many}
  \end{subfigure}
\;
  \begin{subfigure}[t]{0.18\textwidth}
    \includegraphics[width=\textwidth]{Error_synthetic_comparative_sigma200_noutliers2_10mics}
    \caption{Localization error with high noise and 2 outliers}
    \label{fig:Error_synth_high_few}
  \end{subfigure}
\;
  \begin{subfigure}[t]{0.18\textwidth}
    \includegraphics[width=\textwidth]{Error_synthetic_comparative_sigma200_noutliers6_10mics}
    \caption{Localization error with high noise and 6 outliers}
    \label{fig:Error_synth_high_many}
  \end{subfigure}
\;
  \begin{subfigure}[t]{0.18\textwidth}
    \includegraphics[width=\textwidth]{legend}
  \end{subfigure}

  \caption{Algorithm evaluation in synthetic data: Localization error in
    mm (\cite{chan1994simple} is used for
    source position estimation from the optimized TDOA values).}
  \label{fig:Error_comparative_synth}
\end{figure*}


==> figures5-6-v1.tex <==
\label{sec:synth-robust-missing}
\begin{figure*}[!t]
  \centering 
\begin{minipage}{0.75\textwidth}
  \centering 
  \begin{subfigure}[t]{0.3\textwidth}
    \includegraphics[width=\textwidth]{SNR_synthetic_comparative_sigma001_noutliers2_10mics}
    \caption{SNR with low noise and 2 outliers}
    \label{fig:SNR_synth_low_few}
  \end{subfigure}
\;
  \begin{subfigure}[t]{0.3\textwidth}
    \includegraphics[width=\textwidth]{SNR_synthetic_comparative_sigma001_noutliers6_10mics}
    \caption{SNR with low noise and 6 outliers}
    \label{fig:SNR_synth_low_many}
  \end{subfigure}

  \begin{subfigure}[t]{0.3\textwidth}
    \includegraphics[width=\textwidth]{SNR_synthetic_comparative_sigma200_noutliers2_10mics}
    \caption{SNR with high noise and 2 outliers}
    \label{fig:SNR_synth_high_few}
  \end{subfigure}
\;
  \begin{subfigure}[t]{0.3\textwidth}
    \includegraphics[width=\textwidth]{SNR_synthetic_comparative_sigma200_noutliers6_10mics}
    \caption{SNR with high noise and 6 outliers}
    \label{fig:SNR_synth_high_many}
  \end{subfigure}
\end{minipage}\hfill
\begin{minipage}{0.20\textwidth}
  \centering 
  \begin{subfigure}[t]{\textwidth}
    \includegraphics[width=\textwidth]{legend}
  \end{subfigure}
\end{minipage}\hfill
  \caption{Algorithm evaluation in synthetic data: SNR in dB.}
  \label{fig:SNR_comparative_synth}
\end{figure*}

\begin{figure*}[!t]
  \centering 
  \begin{subfigure}[t]{0.23\textwidth}
    \includegraphics[width=\textwidth]{Error_synthetic_comparative_sigma001_noutliers2_10mics}
    \caption{Localization error with low noise and 2 outliers}
    \label{fig:Error_synth_low_few}
  \end{subfigure}
\;
  \begin{subfigure}[t]{0.23\textwidth}
    \includegraphics[width=\textwidth]{Error_synthetic_comparative_sigma001_noutliers6_10mics}
    \caption{Localization error with low noise and 6 outliers}
    \label{fig:Error_synth_low_many}
  \end{subfigure}
\;
  \begin{subfigure}[t]{0.23\textwidth}
    \includegraphics[width=\textwidth]{Error_synthetic_comparative_sigma200_noutliers2_10mics}
    \caption{Localization error with high noise and 2 outliers}
    \label{fig:Error_synth_high_few}
  \end{subfigure}
\;
  \begin{subfigure}[t]{0.23\textwidth}
    \includegraphics[width=\textwidth]{Error_synthetic_comparative_sigma200_noutliers6_10mics}
    \caption{Localization error with high noise and 6 outliers}
    \label{fig:Error_synth_high_many}
  \end{subfigure}
%% \;
%%   \begin{subfigure}[t]{0.18\textwidth}
%%     \includegraphics[width=\textwidth]{legend}
%%   \end{subfigure}

  \caption{Algorithm evaluation in synthetic data: Localization error in
    mm (\cite{chan1994simple} is used for
    source position estimation from the optimized TDOA values). Legend
    is the same as in Fig.~\ref{SNR_synth_high_few}.}
  \label{fig:Error_comparative_synth}
\end{figure*}


==> figures5-6-v2.tex <==
\begin{figure}[!t]
  \centering 
  \includegraphics[width=.25\textwidth]{legend}
  \caption{Legend for Figs.~\ref{fig:SNR_synth_high_many} and~\ref{fig:Error_comparative_synth}.}
  \label{fig:legend}
\end{figure}


\label{sec:synth-robust-missing}
\begin{figure*}[!t]
  \centering 
  \begin{subfigure}[t]{0.23\textwidth}
    \includegraphics[width=\textwidth]{SNR_synthetic_comparative_sigma001_noutliers2_10mics}
    \caption{SNR with low noise and 2 outliers}
    \label{fig:SNR_synth_low_few}
  \end{subfigure}
\;
  \begin{subfigure}[t]{0.23\textwidth}
    \includegraphics[width=\textwidth]{SNR_synthetic_comparative_sigma001_noutliers6_10mics}
    \caption{SNR with low noise and 6 outliers}
    \label{fig:SNR_synth_low_many}
  \end{subfigure}
\;
  \begin{subfigure}[t]{0.23\textwidth}
    \includegraphics[width=\textwidth]{SNR_synthetic_comparative_sigma200_noutliers2_10mics}
    \caption{SNR with high noise and 2 outliers}
    \label{fig:SNR_synth_high_few}
  \end{subfigure}
\;
  \begin{subfigure}[t]{0.23\textwidth}
    \includegraphics[width=\textwidth]{SNR_synthetic_comparative_sigma200_noutliers6_10mics}
    \caption{SNR with high noise and 6 outliers}
    \label{fig:SNR_synth_high_many}
  \end{subfigure}

  %% \begin{subfigure}[t]{\textwidth}
  %%   \includegraphics[width=\textwidth]{legend}
  %% \end{subfigure}

  \caption{Algorithm evaluation in synthetic data: SNR in dB. Legend
    is shown in Fig.~\ref{fig:legend}.}
  \label{fig:SNR_comparative_synth}
\end{figure*}

\begin{figure*}[!t]
  \centering 
  \begin{subfigure}[t]{0.23\textwidth}
    \includegraphics[width=\textwidth]{Error_synthetic_comparative_sigma001_noutliers2_10mics}
    \caption{Localization error with low noise and 2 outliers}
    \label{fig:Error_synth_low_few}
  \end{subfigure}
\;
  \begin{subfigure}[t]{0.23\textwidth}
    \includegraphics[width=\textwidth]{Error_synthetic_comparative_sigma001_noutliers6_10mics}
    \caption{Localization error with low noise and 6 outliers}
    \label{fig:Error_synth_low_many}
  \end{subfigure}
\;
  \begin{subfigure}[t]{0.23\textwidth}
    \includegraphics[width=\textwidth]{Error_synthetic_comparative_sigma200_noutliers2_10mics}
    \caption{Localization error with high noise and 2 outliers}
    \label{fig:Error_synth_high_few}
  \end{subfigure}
\;
  \begin{subfigure}[t]{0.23\textwidth}
    \includegraphics[width=\textwidth]{Error_synthetic_comparative_sigma200_noutliers6_10mics}
    \caption{Localization error with high noise and 6 outliers}
    \label{fig:Error_synth_high_many}
  \end{subfigure}
%% \;
%%   \begin{subfigure}[t]{0.18\textwidth}
%%     \includegraphics[width=\textwidth]{legend}
%%   \end{subfigure}

  \caption{Algorithm evaluation in synthetic data: Localization error in
    mm (\cite{chan1994simple} is used for
    source position estimation from the optimized TDOA values). Legend
    is shown in Fig.~\ref{fig:legend}.}
  \label{fig:Error_comparative_synth}
\end{figure*}


==> figures7-8.tex <==
\begin{figure}[!t]
  \centering 
   \includegraphics[width=0.48\textwidth]{MapSNR_synthetic_comp_ALL_10mics}
  \caption{Missing data recovery in synthetic data: SNR in dB, higher
    is better.}
  \label{fig:MapSNR_synthetic_comp_10mics}
\end{figure}

\begin{figure}[!t]
  \centering 
   \includegraphics[width=0.48\textwidth]{MapCHAN_synthetic_comp_ALL_10mics}
  \caption{Missing data recovery in synthetic data: Localization error
    in mm (using \cite{chan1994simple}), lower is better.}
  \label{fig:MapCHAN_synthetic_comp_10mics}
\end{figure}


==> table-comparison-v1.tex <==
\begin{table*}[t!]
  \renewcommand{\arraystretch}{1.3}
  \caption{Real data performance comparison with selected algorithms in~\cite{alameda2014geometric} ($T_{60}\approx0.5s$)}
  \label{tab:results-real-data2}
  \centering
  \begin{tabular}{l|ccccc|cccc}
    \hline
    &\multicolumn{5}{|c|}{\RobustDenoisingAlg{}}&\multicolumn{4}{c}{Selected algorithms from~\cite{alameda2014geometric}}\\

    &$k=0$  &$k=1$  &$k=2$  &$k=3  $&$k=4$  & \emph{n-mult} & \emph{t-mult}  & \emph{f-mult}      & \emph{b\&b}\\
    \hline
   \% Inliers 
    &23.78\%&24.12\%&25.20\%&25.71\%&23.52\%&13.99\%&17.38\%&17.91\%&27.60\%\\
   Mean angular error of inliers 
    &17.21  &16.44  &16.60  &16.78  &17.66  &17.08  &16.05  &15.25
                            &16.89 \\
   Standard deviation of angular error
    & 7.52  & 7.44  & 7.52  & 7.52  & 7.38  & 7.31  & 7.80  & 7.78
                            &7.50  \\
%    \hline

  \end{tabular}
  % \end{tabular}
\end{table*}

